Towards a Blockchain-based Software Engineering Education

Blockchain technologies for rewards in education are gaining attraction as a promising approach to motivate student learning and promote academic achievement. By providing tangible rewards for educational attainment and engagement, such as digital tokens, educators can motivate learners to take a more active role in their learning and increase their sense of ownership and responsibility for their academic outcomes. In this context, this work proposes the Software Engineering Skill (SES) token as a way of rewarding students in order to improve their experiences in Software Engineering Education (SEE). We performed a proof of concept and conclude that SES token can be deployed in a platform to support SEE.

==> sections/background.tex <==
% Uma cadeia de blocos. Cada bloco tem transações. Transações podem enviar cripto moedas OU transacionar os smart contracts (que são programas que estão na blockchain da rede Ethereum.
% Passos para criar um smart contracts
    % escreve o contrato
    % compila para linguagem de máquina
    % usando um carteira ou enviar direto o programa para um nó da rede e esse nó espalha o programa para todos os nós

% esses programas são disseminados pelo protocolo JSON-RPC (faz a comunicação entre os nós dos blocos)
% existem APIs que facilitam chamadas JSON-RPC
% Web3.js é um framework para usar facilmente o protocolo JSON-RPC

% cada nó é um PC e tem uma cópia da blockchain
% cada nó tem uma implementação do protocolo Ethereum, através de um programa(s)
% esses programas podem ser desenovolvidos na linguagem Go Ethereum, ou Geth
% precisa ter um poder computacional grande para ter uma cópia da blockchain em um nó. Portanto, há possibilidade de usar um nó remoto para fazer interação entre dApp e blockchain.
% existem nós remotos públicos (têm limitações) e privados (exemplo Infura, quicknode, alchemy, moralis)
% para o desenvolvimento, é usado o Ganache para usar um blockchain locamente. 

\section{Blockchain} \label{sec:background}


==> sections/evaluation.tex <==
% result (278125ms) ~ 4,635416667 minutes

\section{Evaluation}

==> sections/relatedwork.tex <==
\section{Related Work}
% \subfile{summary-alammary-2019}

==> sections/ses-code.tex <==
\begin{lstlisting}[language={JavaScript}, caption={SES token code}, label={list:ses-token}]
pragma solidity ^0.8.18;

import "@openzeppelin/contracts/token/ERC20/ERC20.sol";
import "@openzeppelin/contracts/token/ERC20/extensions/ERC20Capped.sol";
import "@openzeppelin/contracts/token/ERC20/extensions/ERC20Burnable.sol";

contract SESkillToken is ERC20Capped {
  address payable public owner;
  uint256 public blockReward;
  
  constructor(uint256 cap, uint256 reward) ERC20("SESkillToken", "SES") ERC20Capped(cap * (10 ** decimals())) {
    owner = payable(msg.sender);
    _mint(owner, 70000000 * (10 ** decimals()));
    blockReward = reward * (10 ** decimals());
  }

  function _mintMinerReward() internal {
    _mint(block.coinbase, blockReward);
  }

  function _beforeTokenTransfer(address from, address to, uint256 value) internal virtual override {
    if(from != address(0) && to != block.coinbase && block.coinbase != address(0)) {
      _mintMinerReward();
    }
    super._beforeTokenTransfer(from, to, value);
  }

  function setBlockReward(uint256 reward) public onlyOwner {
    blockReward = reward * (10 ** decimals());
  }

  function destroy() public onlyOwner {
    selfdestruct(owner);
  }

  modifier onlyOwner {
    require(msg.sender == owner, "Only the owner can call this function");
    _;
  }
}
\end{lstlisting}

==> sections/ses-unit-test-code.tex <==
\begin{lstlisting}[language={Solidity}, caption={SES token unit test}, label={list:ses-token-test}]
it("Should transfer tokens between accounts", async function () {
    await sekillToken.transfer(addr1.address, 50);
    const addr1Balance = await sekillToken.balanceOf(addr1.address);
    expect(addr1Balance).to.equal(50);

    await sekillToken.connect(addr1).transfer(addr2.address, 50);
    const addr2Balance = await sekillToken.balanceOf(addr2.address);
    expect(addr2Balance).to.equal(50);
}
\end{lstlisting}

==> sections/summary-alammary-2019.tex <==
% SUMMARY OF THE WORK
% Blockchain-Based Applications in Education: A Systematic Review
% Ali Alammary * , Samah Alhazmi, Marwah Almasri and Saira Gillani

\textbf{Certificates management}
This category concerns handling all forms of academic credentials, transcripts, students’ certificates, or any other forms of accomplishment records. Most of certificates applications benefited from the high
level of trust and privacy provided by using blockchain technology.
For example, Nespor [7] suggested the development of a blockchain-based certification platform that would provide compensation to schools for their role as certification agents. This proposed application would grant higher education providers or employers the authority to issue official certificates to students while maintaining a high level of privacy for their personal information. Consequently, students would be able to share their official documents with interested parties directly, without the need for intermediaries.

\textbf{Competencies and learning outcomes management}
Considerable emphasis has been placed on developing blockchain applications that can enhance learning objectives and foster the acquisition of competencies in educational settings. These applications have the potential to improve the learning process and expand the educational domain across a broad range of disciplines. Given the inherent efficiency of blockchain technology, these applications can effectively assess and evaluate student performance based on qualitative and quantitative metrics.
For example, For instance, Farah, Vozniuk, Rodríguez-Triana and Gillet [22] developed a system for tracking student performance across multiple learning activities. The system aggregates individual traces of each activity into a block, which can be considered self-describing due to the inclusion of metadata for numerous activities. This approach has the potential to greatly enhance the overall self-efficiency of the system.

\textbf{Securing a collaborative learning environment}
This category pertains to the importance of utilizing blockchain technology to facilitate the learning environment. The decentralized network offered by blockchain enables easy access with high levels of security and integrity, fostering a collaborative atmosphere among all stakeholders, including students, faculty members, and authorities. As an example, the authors in Reference [30] presented a system, which employs blockchain technology to offer students a secure collaborative learning environment that can be accessed at any time and from anywhere.

% 4????

\textbf{Fees and credits transfer}
This category discusses applications with similar features that leverage blockchain technology for the secure and trustworthy transfer of credential records or fees among institutions, organizations, and universities. Typically, educational institutions depend on intermediaries to handle and approve the transfer of credits or fees. However, the high-security level of blockchain presents an efficient alternative that can eliminate the need for such intermediaries. For instance, the EduCTX system [34] utilizes tokens to facilitate the transfer process. These tokens can represent any form of a digital learning unit, such as certificates, courses, and diplomas. Each educational institution has its own EduCTX address, enabling them to manage the transfer process in a secure manner.

\textbf{Obtaining digital guardianship consent}
Blockchain technology has enabled the traditional process of obtaining parental consent to be replaced by electronic means, owing to the high level of trust it provides. The decentralized nature of blockchain facilitates the swift collection of consent while ensuring privacy is not compromised. This has a significant impact on streamlining the process of collecting and communicating consent across a large number of students, parents, and educational institutions. Gilda and Mehrotra [36] proposed a framework that enables public schools to grant authorization rights to third-party institutions without requiring parental consent for each interaction. The use of blockchain technology in this framework establishes a nested authorization process that expedites the entire process while guaranteeing privacy and access control of consent.

\textbf{Competition management}
This category leverages blockchain technology to simplify the management of competition operations and improve its efficiency and transparency. Wu and Li [29] presented a competition model that is based on an e-commerce operation sandbox, which is a decision-making system that evaluates students' professional knowledge and expertise. They developed this system to create an evaluation mechanism that measures and manages the operational proficiency of students.

\textbf{Evaluating students’ professional ability}
Assessing the professional capabilities of students is another category that establishes a connection between students' professionalism and specific industries to provide employment recommendations. Liu, Guan, Yang, Zhu, Green, and Yin [26] conducted a study in this category, which employed blockchain technology to establish a link between educational institutions and employment enterprises for sharing all the necessary information regarding recruitment and industry requirements.

\textbf{Copyrights management}
The management of copyrights is crucial in maintaining ownership rights, and blockchain technology offers a promising solution for this purpose. Hori et al. (2018) presented the implementation of a decentralized learning system, known as "CHiLO," which leverages blockchain to safeguard the copyrights and ownerships of e-books. Another category that highlights the significance of blockchain in education is the protection of learning objects. By utilizing blockchain applications, students and faculty members can protect any newly acquired knowledge or learning objects.

\textbf{students’ interactions in the e-learning}
Another application category that leverages blockchain technology is enhancing students' interactions in e-learning systems. This category aims to address issues related to student's engagement in the e-learning environment. Zhong, Xie, Zou, and Chui [32] proposed a potential blockchain-based application designed to improve learning engagement by providing rewards in the form of virtual currencies to top-ranked learners. The application utilizes predefined policies deployed on the blockchain network to determine the reward distribution.

\textbf{Examination review}
Examination review is another application category of blockchain applications in education. 
The use of permissioned blockchain technology is proposed to enhance the security of auditing exam papers through the use of trusted ledgers. Mitchell, Hara, and Sheriff [38] developed a decentralized application for examination review called "dAppER" that adheres to quality assurance standards by distributing exam papers among external examiners.

\textbf{lifelong learning}
The final category of blockchain application is supporting lifelong learning, which involves using blockchain technology to enhance skills, knowledge, and efficiency for learners. Mikroyannidis et al. [39] discussed the impact of blockchain on real-life learning and presented an ecosystem that places the learner at the center of the learning process and its associated data. The authors highlighted how accreditation, tutoring, and ePortfolios can be developed within this lifelong learning ecosystem using blockchain technology. The proposed model empowers learners to create an effective plan for their educational journey based on their desired career trajectory, providing them with complete control and ownership during the learning process.

==> sections/summary-dapp-education.tex <==
\section{dApp for Education}

\subsection{Uma aplicação descentralizada (dApp) para educação pode recompensar seus usuários por meio de tokens por meio de diferentes abordagens. Aqui estão algumas ideias:}

\begin{enumerate}
    \item Sistema de pontuação: A aplicação pode atribuir pontos a um usuário sempre que ele concluir uma tarefa ou atividade, como assistir a um vídeo educacional ou responder a uma pergunta. Esses pontos podem ser convertidos em tokens, que podem ser usados para desbloquear recursos adicionais ou recursos premium na aplicação.
    \item Recompensas por conclusão de cursos: A aplicação pode oferecer tokens como recompensa para usuários que concluírem cursos ou módulos inteiros. Isso pode incentivar os usuários a concluir seus estudos e melhorar a sua compreensão do assunto.
    \item Contribuições da comunidade: A aplicação pode incentivar a participação da comunidade, permitindo que os usuários criem conteúdo, contribuam com ideias ou ajudem outros usuários. Essas contribuições podem ser recompensadas com tokens, incentivando a colaboração e a criação de uma comunidade forte.
    \item Gamificação: A aplicação pode adicionar elementos de jogos para tornar o aprendizado mais envolvente e divertido. Os usuários podem receber tokens por alcançar certos marcos, completar desafios ou ganhar competições.
\end{enumerate}

É importante lembrar que a distribuição de tokens deve ser cuidadosamente planejada para evitar abusos ou fraudes. A aplicação pode usar contratos inteligentes para automatizar a distribuição de tokens e garantir que todos os usuários sejam recompensados de forma justa e transparente. Além disso, a aplicação deve fornecer uma maneira fácil para os usuários trocarem os tokens por outras criptomoedas ou moedas fiduciárias, se desejarem.

\subsection{Uma aplicação descentralizada de educação pode utilizar tokens de várias maneiras para engajar o ensino e incentivar a participação da comunidade. Alguns exemplos incluem:}

\begin{enumerate}
    \item Recompensas por participação: a aplicação pode recompensar os usuários com tokens por sua participação em fóruns de discussão, grupos de estudo, respostas a perguntas ou comentários em postagens. Isso incentiva a participação da comunidade e ajuda a criar um ambiente de aprendizado colaborativo.
    \item Recompensas por conclusão de cursos: a aplicação pode oferecer tokens aos usuários que concluírem com sucesso um curso ou módulo. Isso ajuda a motivar os usuários a concluir os cursos e pode incentivar a aquisição de habilidades.
    \item Recompensas por contribuições: a aplicação pode oferecer tokens para usuários que contribuem com conteúdo educacional de alta qualidade, como vídeos, textos ou exercícios. Isso incentiva a criação e compartilhamento de recursos educacionais úteis.
    \item Pagamento de taxas de curso: os usuários podem usar tokens para pagar por taxas de curso ou outros recursos adicionais. Isso torna o processo de pagamento mais fácil e seguro, além de oferecer uma opção adicional de pagamento.
    \item Troca de tokens: os usuários podem trocar tokens por outras criptomoedas ou bens e serviços no mercado. Isso pode ajudar a criar um ecossistema econômico em torno da aplicação de educação descentralizada, incentivando a adoção e o uso contínuo da plataforma.
\end{enumerate}

Essas são apenas algumas maneiras pelas quais a utilização de tokens pode ser utilizada em uma aplicação descentralizada de educação para incentivar o engajamento e a participação da comunidade. A tecnologia blockchain permite a criação de um sistema seguro e transparente para a distribuição de tokens, tornando a aplicação mais eficiente e confiável.

==> sections/summary-tokens.tex <==
From: https://www.infomoney.com.br/guias/tokens/

\section{Tipos de token}
A todo o momento, o mercado cria novos tipos de tokens, com propostas, sabores e nomes variados. No geral, no entanto, é possível dividi-los em quatro categorias principais.

\textbf{Payment Tokens}
Os Payment tokens são utilizados para transferência de capital, funcionando como dinheiro eletrônico. O Bitcoin, o Ethereum e boa parte das mais de 10 mil criptomoedas existentes no mercado se enquadram nessa categoria.

\textbf{Utility tokens}
Os Utility tokens oferecem alguma utilidade, como desconto em um produto específico ou acesso a um serviço exclusivo. Os fan tokens, ativos digitais de clubes de futebol, são exemplos. Alguns times dão aos detentores o direito de votar em enquetes, escolher a frase a ser escrita em alguma dependência do estádio, participar de promoções ou ter acessos exclusivos a locais.

\textbf{Non-fungible tokens (NFT)}
Non-fungible tokens (NFT) ou tokens não-fungíveis – são tokens que representam algo único. Eles podem “espelhar” obras de arte, músicas, capas históricas de revistas e até tweets. Ao adquirir um NFT, a pessoa basicamente compra um código de computador que contém o registro do objeto.

\textbf{Security tokens}
Os Security tokens representam algum valor imobiliário, como uma ação negociada na Bolsa de Valores. Como estão “ligados” a produtos regulados, eles precisam atender às regras de supervisores do mercado de capitais.

\section{Diferença entre token e criptomoedas}
Toda criptomoeda é um token, mas nem todo token é uma criptomoeda, segundo Rafael Nasser, professor doutor em Informática da PUC-Rio. De acordo com ele, o BTC seria o token da rede Bitcoin, enquanto o ETH seria o token da blockchain do Ethereum.

\section{Como funciona?}
O funcionamento do token depende do projeto e da categoria na qual o ativo se enquadra. No geral, no entanto, eles “rodam” em alguma blockchain. Além disso, são baseados em contratos inteligentes.

Os payments tokens funcionam como meio de pagamento. Os utility tokens, por outro lado, dão acesso a serviços exclusivos, cupons de descontos, direito a voto e outros benefícios.

Já os NFTs (sigla em inglês para tokens não-fungíveis) representam algo único – portanto, são itens virtuais colecionáveis exclusivos. O security token, por fim, é semelhante a valores mobiliários, como ações, e dão direito a lucro. 


==> sections/summary-zhong-2018.tex <==
% SUMMARY OF THE WORK
% A Blockchain Model for Word-Learning Systems
% Jiemin Zhong, Haoran Xie, Di Zou

B. The potential applications of blockchain
Virtual currency as a learning reward. 
As shown in Figure 2, each user has a unique ETH address as an identity. Learners can earn credits when they participate in community activities, and the credits can be converted into the virtual currency. These virtual currencies can be used to purchase some paid or encrypted files, which can avoid plagiarism and protect the intellectual property of owners. To improve learning engagement, the system can give an
extra reward to the top-ranked learners based on incentive policies that can be deployed on the blockchain.
